Code-as-Monitor: Constraint-aware Visual Programming for Reactive and Proactive Robotic Failure Detection

Automatic detection and prevention of open-set failures are crucial in closed-loop robotic systems. Recent studies often struggle to simultaneously identify unexpected failures reactively after they occur and prevent foreseeable ones proactively. To this end, we propose Code-as-Monitor (CaM), a novel paradigm leveraging the vision-language model (VLM) for both open-set reactive and proactive failure detection. The core of our method is to formulate both tasks as a unified set of spatio-temporal constraint satisfaction problems and use VLM-generated code to evaluate them for real-time monitoring. To enhance the accuracy and efficiency of monitoring, we further introduce constraint elements that abstract constraint-related entities or their parts into compact geometric elements. This approach offers greater generality, simplifies tracking, and facilitates constraint-aware visual programming by leveraging these elements as visual prompts. Experiments show that CaM achieves a 28.7% higher success rate and reduces execution time by 31.8% under severe disturbances compared to baselines across three simulators and a real-world setting. Moreover, CaM can be integrated with open-loop control policies to form closed-loop systems, enabling long-horizon tasks in cluttered scenes with dynamic environments.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec: intro}
\clearpage
%
% The ability to detect execution failures and recover automatically during long-horizon open-world tasks is crucial for a closed-loop robotic system.
% %
% However, achieving this requires robots to deeply understand the complex physical world and free-form human instructions, while accurately detecting failure in real-time and re-planning accordingly.
% %
 
% Failure detection has advanced rapidly with the development of large language models~(LLMs)~\cite{dubey2024llama, touvron2023llama} and vision-language models~(VLMs)~\cite{achiam2023gpt, liu2024visual}.
% %
% Previous methods~\cite{liu2023reflect, shinn2023reflexion, yao2022react, ha2023scaling, huang2022inner, silver2024generalized, skreta2023errors, raman2022planning} convert visual inputs into textual descriptions of entities (\eg, target objects, robot end effectors) in the environment and rely on LLMs for failure detection, but often miss fine-grained entity state details.
% %
% Leveraging VLMs' powerful visual understanding, several studies~\cite{du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer} analyze final visual outcomes after task completion to detect failures but overlook them during execution.
% %
% % neglect the misalignment between planning and execution when failures occur during the task.
% %
% Recent works~\cite{guo2023doremi, yu2023multireact} frequently query VLMs for failure detection during execution. Yet, two key challenges remain: 1) detection isn't \textit{real-time} due to the VLMs' high computational cost, and 2) it lacks \textit{precision}, as VLMs have limited 3D spatial understanding and frequent querying VLMs increases hallucination risks.
% %

% %
% To this end, we introduce Constraint-aware Visual Programming~({\fname}), a novel paradigm leveraging VLMs for \textit{real-time} and \textit{precise} failure detection and recovery.
% %
% Our key idea is to use VLMs to generate monitor code, enabling \textit{real-time} checks on spatiotemporal constraints between entities (\eg, robots, object parts) during execution.
% %
% By computing the entity states and reducing the frequency of VLM queries~(\ie, generating code once per subgoal), {\fname} improves \textit{precision} and mitigates hallucinations.
% %
% Direct visual programming from raw images remains challenging for VLMs, as it involves encoding both spatiotemporal states of entities and their constraints.
% %
% Thus, {\fname} is decomposed into two modules, as shown in \todo{\cref{xxx}}.
% %
% The first Painter, based on the current observations (\ie, multi-view RGB-D observations) and subgoals, generates textual constraints that are then annotated onto the images as constraint elements~(\eg, points, lines, surfaces), represented by 3D points in the world frame.
% %
% The second Monitor employs a VLM (\eg, GPT-4o~\cite{achiam2023gpt}) to translate these annotated images into monitor code that specifies the state entities must maintain during and after subgoal execution.
% %
% It then continuously tracks the 3D points of the constraint elements in real-time, executing the monitor code for immediate failure detection during execution.




% Notably, the Painter can autonomously generate constraint elements.
% %
% Specifically, our trained model performs constraint-aware part segmentation across multi-view images for each constraint. The segmented parts are then lifted to 3D space, with a representative 3D point selected from each part's point cloud. These points are then connected to form the final element of one constraint.
% %
% Compared to directly training a 3D part segmentation model, we can leverage more 2D image data for training, resulting in more accurate and generalizable performance.


% %
% We conduct extensive experiments in three simulators~(\ie, CLIPort, Omnigibson, and RLBench) and one real-world setting, spanning diverse manipulation tasks (\eg, pick \& place, articulated objects), robot platforms (\eg, UR5, Franka, Fetch) and end-effectors (\eg, suction cup, gripper, dexterous hand).
% %
% The results show that {\fname} is generalizable and achieves more \textit{real-time} and \textit{precise} failure detection and recovery compared to the baseline methods, resulting in significantly higher success rates (xxx times) and reduced execution times (xxx times).
% %
% Moreover, in \todo{\cref{xxx}}, {\fname} can be extended to function as a monitor, enabling closed-loop planning in cluttered scenes.
% %
% Our contributions are summarized as follows:
% \begin{itemize}
%     \item We introduce constraint-aware visual programming, {\fname}, a novel paradigm that leverages VLM for \textit{real-time}, \textit{precise} robotic failure detection and recovery.
%     \item We propose a 2D constraint-aware part segmentation model to effectively help generate constraint elements for producing more accurate monitor code.
%     \item Experiments show that {\fname} is generalizable and achieves more \textit{real-time} and \textit{precise} failure detection compared to baseline methods. 
% \end{itemize}




% \vspace{-4mm}
\section{Introduction}
\label{sec: intro}
% \clearpage
%
% Automatically preventing and detecting execution failures is crucial for closed-loop robotic systems performing long-horizon, open-world tasks.
%
As expectations grow for robots to handle long-horizon tasks within intricate environments, failures are unavoidable. 
%
% Therefore, it is vital for robotic systems to detect and prevent those failures automatically in a closed-loop manner. 
%
Therefore, automatically detecting and preventing those failures are of vital role in ensuring the tasks can be eventually solved, especially for closed-loop robotic systems.
%
There are two modes of failure detection~\cite{lemasurier2024reactive}, \textit{reactive} and \textit{proactive}. 
% 
As depicted in \cref{fig: motivation}, \textit{reactive} failure detection aims to identify failures after they occur~(\eg, recognizing that lobster lands on the table, \textit{indicating} a delivery failure).
%
In contrast, \textit{proactive} failure detection aims to prevent foreseeable failures~(\eg, recognizing that a tilted pan could lead to the lobster falling out, \textit{leading to} a delivery failure).
%
Both detection modes are even more challenging in open-set scenarios, where the failures are not predefined.
%


% Recent studies primarily focus on \textit{reactive} failure detection~\cite{huang2022inner, silver2024generalized, skreta2023errors, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer, guo2023doremi, yu2023multireact}, 
% with the help of large language models~(LLMs)~\cite{dubey2024llama, touvron2023llama} or vision-language models~(VLMs)~\cite{achiam2023gpt, liu2024visual} to identify failures after they occur, in the form of visual question-answering~(VQA). 
%
% These methods relax real-time performance and precision requirements, aligning with LLMs/VLMs' inherent limitations such as high computational cost and inadequate 3D spatio-temporal understanding.
With the help of large language models~(LLMs)~\cite{dubey2024llama, touvron2023llama} or vision-language models~(VLMs)~\cite{achiam2023gpt, liu2024visual}, recent studies can achieve open-set \textit{reactive} failure detection~\cite{huang2022inner, silver2024generalized, skreta2023errors, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer, guo2023doremi, yu2023multireact}, as a special case of visual question-answering~(VQA) tasks. 
%
However, these methods often bear compromised execution speeds and coarse-grained detection accuracy, due to the high computational costs and inadequate 3D spatio-temporal perception capability of recent LLMs/VLMs.
%
% But recent LLMs/VLMs' limitations such as high computational costs and inadequate 3D spatio-temporal perception capability, 
%
Conversely, open-set \textit{proactive} failure detection, which has been less explored in the literature, presents even severer challenges as it is required to foresee potential causes of failure and monitor them in real-time with high precision to anticipate and prevent imminent failure.
%
Simply adapting LLMs/VLMs cannot meet such expectations.

%
% In this work, we aim to study how to use a generalized modeling approach to achieve both challenging proactive and reactive failure detection. 
%
In this work, we aim to develop an open-set failure detection framework that achieves reactive and proactive detection simultaneously, not only benefiting from the generalization power of VLMs but also enjoying high precision in monitoring failure characteristics with real-time efficiency. 
%
We address this by formulating both tasks as a unified set of spatio-temporal constraint satisfaction problems, which can be \emph{precisely} translated by VLMs into executable programs.
%
Such visual programs can efficiently verify whether entities (\eg, robots, objects) or their parts in the captured environment maintain or achieve required states during or after execution (\ie, satisfying constraints), so as to \emph{immediately} prevent or detect failures.
%
To the best of our knowledge, this is the first attempt to integrate both detection modes within a single framework.
%
We name this constraint-aware visual programming framework as Code-as-Monitor~({\fname}).
%
% To enable real-time and precise constraint checking, we leverage VLMs for automatically generating code to compute inter-entity constraints and monitor their fulfillment, naming the framework Code-as-Monitor~({\fname}).




% To be specific, the proposed spatio-temporal constraint computation is designed to replace naively applying costly and unreliable VLMs.
%
To be specific, the proposed spatio-temporal constraint satisfaction scheme abstracts the constraint-related entity or part segments from the observed images into compact geometric elements (\eg, points, lines, and surfaces), as shown in \cref{fig: motivation}.
%
It simplifies the monitoring of constraint satisfaction by tracking and evaluating the spatio-temporal combinational dynamics of these elements, eliminating the most irrelevant geometric and visual details of the raw entities/parts.
%
The constraint element detection and tracking are grounded by our trained constraint-aware segmentation and off-the-shelf tracking models, ensuring speed, accuracy, and certain open-set adaptation capabilities.
%
The evaluation protocol is in the form of VLM-generated code, \ie, monitor code, which is visually prompted by the starting frames of a sub-goal and its associated constraint elements, in addition to the textual constraints that must be fulfilled. 
%
Once generated, this monitor code could detect reactive or proactive failures just by being executed according to the tracked constraint elements, without needing to call the VLMs again.
%
Therefore, this minimalist scheme is generalizable to open-set failure detection with unseen scenes and entities (enabled by the potential diversity of the structured associations of constraint elements) and common skills (powered by the rich prior knowledge offered by VLMs), with sufficient detection accuracy and real-time execution speed. 

%
% These elements are annotated onto observed images~(see \cref{fig: motivation}~(c)) 

% To enhance the accuracy and efficiency of the constraint computation, we introduce constraint elements (\eg, points, lines, surfaces) by abstracting constraints as relationships between entities or their parts, further simplifying them into compact, combinable units while retaining their inherent constraint properties.
% %
% These elements are annotated onto images~(see \cref{fig: motivation}~(c)) for visual programming and continuously tracked during execution for code computation.
% %
% The elements enable more precise tracking and facilitate simpler code generation and computation than directly handling the constraint-related objects or their parts.
% %
% It is the key enabler to achieve \textit{proactive} failure detection.
% %
% Moreover, representing constraints as relationships between entities or parts provides generalizability, allowing the compression of parts into elements to extend to common scenarios and objects.




% %
% By abstracting constraints into relations of entity-related parts and compressing these parts into fundamental elements while preserving information density, we enable more precise tracking and simpler code generation and computation compared to directly tracking objects or parts. 
% %
% %


% To improve the precision of constraint computation, we design two modules in {\fname}, \ie, the Painter and Monitor.
% First, we leverage the painter to accurately extract the constraint elements~(\eg, points, lines, surfaces) and overlay them onto the image, as shown in the \cref{fig: motivation}~(c).
% Instead of directly using the raw image for visual programming, we use the painter’s output as a visual prompt to improve precision.
% %
% % The Painter converts the textual constraints and current observations (\ie, multi-view RGB-D data) into constraint element proposals~(\eg, points, lines, surfaces) represented by 3D points and then annotated onto the images, as shown in the \cref{fig: motivation}~(c).
% %
% Notably, we train a multi-granularity constraint-aware segmentation model to obtain the constraint-related objects and parts, which can be lifted to 3D space using depth and better form the desired elements.
% %
% % Then the desired 3D points are selected from each part's point clouds to form the final elements compared to directly relying on 3D part segmentation models.
% %
% Second, the Monitor then translates these annotated images into monitor code and tracks these element positions in real-time, executing the code for both \textit{reactive} and \textit{proactive} failure detection.



%
We conduct extensive experiments in three simulators~(\ie, CLIPort~\cite{shridhar2021cliport}
, Omnigibson~\cite{li2022behavior}, and RLBench~\cite{james2019rlbench}) and one real-world setting, spanning diverse manipulation tasks (\eg, pick \& place, articulated objects), robot platforms (\eg, UR5, Fetch, Franka) and end-effectors (\eg, suction cup, gripper, dexterous hand).
%
The results show that {\fname} is generalizable and achieves both \textit{reactive} and \textit{proactive} failure detection in real-time, resulting in $29\%$ higher success rates and reduced execution time by $33\%$ under severe disturbances compared to the baseline methods.
%
Moreover, in \cref{subsec: main results in real world}, {\fname} can be surprisingly integrated with the existing open-loop control policy to form a closed-loop system, enabling long-horizon tasks in cluttered scenes with environment dynamics and human disturbance.
%
Our contributions are summarized as follows:
\begin{itemize}
    \item We introduce Code-as-Monitor~(\fname), a novel paradigm that leverages VLMs for both \textit{reactive} and \textit{proactive} failure detection via constraint-aware visual programming.
    \item We propose the constraint elements to enhance the accuracy and efficiency of constraint satisfaction monitoring.
    \item Extensive experiments show that {\fname} is generalizable and achieves more real-time and precise failure detection than baselines across simulators and real-world settings. 
\end{itemize}

==> sec/1_intro_v2.tex <==
\section{Introduction}
\label{sec: intro}
\clearpage
%
% Automatically preventing and detecting execution failures is crucial for closed-loop robotic systems performing long-horizon, open-world tasks.
%
Automatically detecting and preventing execution failures is crucial for closed-loop robotic systems performing long-horizon, open-world tasks.
%
Thus, such robots require both \textit{reactive} and \textit{proactive} failure detection~\cite{lemasurier2024reactive}, as shown in \cref{fig: motivation}.
%
Specifically, the \textit{reactive} failure detection focuses on identifying failures after they have occurred~(\eg, recognizing that a piece of bread has fallen onto the table during transfer, \textit{indicating} a delivery failure).
%
In contrast, the \textit{proactive} failure detection aims to prevent potential failures caused by environmental dynamics or imperfect action execution (\eg, recognizing that a tilted pan could lead to the bread falling out, \textit{leading to} a delivery failure).
%

%
Recent works leverage vision-language models~(VLMs) \cite{achiam2023gpt, liu2024visual} to achieve open-set \textit{reactive} failure detection by either querying VLMs for post-execution detection~\cite{liu2023reflect, shinn2023reflexion, yao2022react, ha2023scaling, huang2022inner, silver2024generalized, skreta2023errors, raman2022planning, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer} but overlooking failures occurring during the process, or frequent querying VLMs during execution~\cite{guo2023doremi, yu2023multireact}.
%
However, two major challenges of \textit{reactive} failure detection remain: (1) detection isn't real-time due to the VLMs' high computational cost during execution, and (2) it lacks precision, as VLMs exhibit limited 3D spatial understanding and frequent querying increases hallucination risks.
%
Furthermore, these VLM-based works rarely explore the \textit{proactive} failure detection, which also should be real-time and precise.



% However, existing research mainly focuses on \textit{reactive} failure detection (\ie, identifying failures after they occur) while largely neglecting \textit{proactive} failure detection (\ie, preventing potential failures), as depicted in \todo{\cref{xxx}}, which hinders the achievement of the desired ability.
%


%
% However, achieving this requires the robot to deeply understand the complex physical world and free-form human instructions, while accurately monitoring itself and the environment in real-time.
%

% Failure detection has advanced rapidly with the development of large language models~(LLMs)~\cite{dubey2024llama, touvron2023llama} and vision-language models~(VLMs)~\cite{achiam2023gpt, liu2024visual}.
% %
% Previous methods~\cite{liu2023reflect, shinn2023reflexion, yao2022react, ha2023scaling, huang2022inner, silver2024generalized, skreta2023errors, raman2022planning, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer} employ LLMs with auxiliary vision modules or VLMs as post-execution failure detectors, neglecting in-execution detection.
% %
% To address this gap, recent works~\cite{guo2023doremi, yu2023multireact} frequently query VLMs during execution for failure detection. However, two major challenges remain: 1) detection isn't real-time due to the VLMs' high computational cost, and 2) it lacks precision, as VLMs exhibit limited 3D spatial understanding and frequent querying increases hallucination risks.
% %
% Moreover, these methods are reactive rather than proactive, detecting failures only after they occur and unable to prevent those arising from environmental changes or task modifications.
% %
% In this work, we study how to effectively endow robots with the ability to solve novel manipulation tasks specified by free-form language instructions using VLMs

%




To this end, we introduce Code-as-Monitor~({\fname}), a novel paradigm leveraging VLMs for both \textit{reactive} and \textit{proactive} failure detection via constraint-aware visual programming.  
%
Our key idea involves two parts: 
%
(1) We formulate \textit{reactive} and \textit{proactive} failure detection as generalized spatio-temporal constraint satisfaction, which involves checking if entities~(\eg, robots, object parts) in the scene maintain or reach the required states during or after execution, to prevent and detect failures. 
%
(2) We employ the VLM-generated monitor code to compute inter-entity constraints in real-time, which reduces VLM calls~(\ie, generating code once per subgoal), thus minimizing hallucinations.

%
Since direct visual programming from raw images and continuous monitoring remains challenging for VLMs, {\fname} is decomposed into two modules, \ie, the Painter and Monitor.
%
The Painter converts the textual constraints and current observations (\ie, multi-view RGB-D data) into constraint element proposals~(\eg, points, lines, surfaces) represented by 3D points and then annotated onto the images, as shown in the \cref{fig: motivation}~(c).
%
Notably, we enhance proposal precision by training a multi-granularity constraint-aware segmentation model to obtain the constraint-related objects and parts, which can be lifted to 3D space using depth and better form the desired elements.
%
% Then the desired 3D points are selected from each part's point clouds to form the final elements compared to directly relying on 3D part segmentation models.
%
The Monitor then translates these annotated images into monitor code and tracks these element positions in real-time, executing the code for both \textit{reactive} and \textit{proactive} failure detection.
%


%

% %
% Our key idea is to use VLMs to generate monitor code, enabling real-time checks on spatiotemporal constraints between entities (\eg, robots, object parts) during execution.
% %
% By computing the entity states and reducing the frequency of VLMs queries~(\ie, generating code once per subgoal), {\fname} improves precision and mitigates hallucinations.
%


% Direct visual programming from raw images remains challenging for VLMs, as it involves encoding both spatiotemporal states of entities and their constraints.
% %
% Thus, {\fname} is decomposed into two modules, as shown in \todo{\cref{xxx}}.
% %
% The first Painter, based on the current observations (\ie, multi-view RGB-D observations) and subgoals, generates textual constraints that are then annotated onto the images as constraint elements~(\eg, points, lines, surfaces), represented by 3D points in the world frame.
% %
% The second Monitor employs a VLMs (\eg, GPT-4o~\cite{achiam2023gpt}) to translate these annotated images into monitor code that specifies the state entities must maintain during and after subgoal execution.
% %
% It then continuously tracks the 3D points of the constraint elements in real time, executing the monitor code for immediate failure detection during execution.




% Notably, the Painter can autonomously generate constraint elements.
% %
% Specifically, our trained model performs constraint-aware part segmentation across multi-view images for each constraint. The segmented parts are then lifted to 3D space, with a representative 3D point selected from each part's point cloud. These points are then connected to form the final element of one constraint.
% %
% Compared to directly training a 3D part segmentation model, we can leverage more 2D image data for training, resulting in more accurate and generalizable performance.


%
We conduct extensive experiments in three simulators~(\ie, CLIPort~\cite{shridhar2021cliport}
, Omnigibson~\cite{li2022behavior}, and RLBench~\cite{james2019rlbench}) and one real-world setting, spanning diverse manipulation tasks (\eg, pick \& place, articulated objects), robot platforms (\eg, UR5, Franka, Fetch) and end-effectors (\eg, suction cup, gripper, dexterous hand).
%
The results show that {\fname} is generalizable and achieves both \textit{reactive} and \textit{proactive} failure detection in real-time, resulting in significantly higher success rates and reduced execution times compared to the baseline methods.
%
Moreover, {\fname} can quickly prevent potential failure caused by environment dynamics and human disturbance, enabling closed-loop planning in cluttered scenes.
%
Our contributions are summarized as follows:
\begin{itemize}
    \item We introduce Code-as-Monitor~(\fname), a novel paradigm that leverages VLMs for both \textit{reactive} and \textit{proactive} failure detection via constraint-aware visual programming.
    \item We propose a multi-granularity constraint-aware segmentation model to help obtain more precise constraint elements for generating more accurate monitor code.
    \item Extensive experiments show that {\fname} is generalizable and achieves more real-time and precise failure detection than baseline methods. 
\end{itemize}

==> sec/1_intro_v3.tex <==
\section{Introduction}
\label{sec: intro}
\clearpage
%
% Automatically preventing and detecting execution failures is crucial for closed-loop robotic systems performing long-horizon, open-world tasks.
%
As expectations grow for robots to handle long-horizon tasks within intricate environments, failures are unavoidable. Therefore, it is vital for robotic systems to detect and prevent those failures automatically in a closed-loop manner. 
%
There are two modes of failure detection~\cite{lemasurier2024reactive}, \textit{reactive} and \textit{proactive}. 
% 
As depicted in \cref{fig: motivation}, \textit{reactive} failure detection aims to identify failures after they have occurred~(\eg, recognizing that bread has fallen onto the table, \textit{indicating} a delivery failure).
%
In contrast, \textit{proactive} failure detection aims to prevent foreseeable failures~(\eg, recognizing that a tilted pan could lead to the bread falling out, \textit{leading to} a delivery failure).
%
Both detection modes are crucial.
%

%
% Taking \cref{fig: motivation} as an example, \textit{reactive} failure detection focuses on identifying failures after they have occurred~(\eg, recognizing that bread has fallen onto the table during transfer, \textit{indicating} a delivery failure).

%
Recent works focus more on leveraging the generalization and reasoning abilities of large language models~(LLMs)~\cite{dubey2024llama, touvron2023llama} or vision-language models~(VLMs) \cite{achiam2023gpt, liu2024visual} for open-set reactive failure detection~\cite{liu2023reflect, shinn2023reflexion, yao2022react, ha2023scaling, huang2022inner, silver2024generalized, skreta2023errors, raman2022planning, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer, guo2023doremi, yu2023multireact}.
%
However, two major challenges of \textit{reactive} failure detection remain: (1) detection isn't real-time due to the VLMs' high computational cost during execution, and (2) it lacks precision, as VLMs exhibit limited 3D spatial understanding and frequent querying increases hallucination risks.
% 
Furthermore, these VLM-based works rarely explore the \textit{proactive} failure detection.
%


Recent works leverage vision-language models~(VLMs) \cite{achiam2023gpt, liu2024visual} to achieve open-set \textit{reactive} failure detection by either querying VLMs for post-execution detection~\cite{liu2023reflect, shinn2023reflexion, yao2022react, ha2023scaling, huang2022inner, silver2024generalized, skreta2023errors, raman2022planning, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer} but overlooking failures occurring during the process, or frequent querying VLMs during execution~\cite{guo2023doremi, yu2023multireact}.
%
However, two major challenges of \textit{reactive} failure detection remain: (1) detection isn't real-time due to the VLMs' high computational cost during execution, and (2) it lacks precision, as VLMs exhibit limited 3D spatial understanding and frequent querying increases hallucination risks.
%
Furthermore, these VLM-based works rarely explore the \textit{proactive} failure detection, which also should be real-time and precise.


Recent work leverages the generalization and reasoning abilities of large language models~(LLMs) \cite{ouyang2022training} or vision-language models~(VLMs) \cite{achiam2023gpt, liu2024visual} for open-set reactive failure detection~\cite{liu2023reflect, shinn2023reflexion, yao2022react, ha2023scaling, huang2022inner, silver2024generalized, skreta2023errors, raman2022planning, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer, guo2023doremi, yu2023multireact}, but overlooking proactive failure detection. 
The primary reasons are twofold. First, the high computational cost hinders real-time detection and intervention before failure occurs. 
Second, taking textual scene descriptions or visual observations as input, LLMs/VLMs struggle to capture detailed information and lack robust 3D spatial understanding, limiting their precision in preventing imminent failures.
%
% Recent works leverage vision-language models~(VLMs) \cite{achiam2023gpt, liu2024visual} to achieve open-set \textit{reactive} failure detection by either querying VLMs for post-execution detection~\cite{liu2023reflect, shinn2023reflexion, yao2022react, ha2023scaling, huang2022inner, silver2024generalized, skreta2023errors, raman2022planning, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer} but overlooking failures occurring during the process, or frequent querying VLMs during execution~\cite{guo2023doremi, yu2023multireact}.
%
% However, two major challenges of \textit{reactive} failure detection remain: (1) detection isn't real-time due to the VLMs' high computational cost during execution, and (2) it lacks precision, as VLMs exhibit limited 3D spatial understanding and frequent querying increases hallucination risks.
%
% Furthermore, these VLM-based works rarely explore the \textit{proactive} failure detection, which also should be real-time and precise.



% However, existing research mainly focuses on \textit{reactive} failure detection (\ie, identifying failures after they occur) while largely neglecting \textit{proactive} failure detection (\ie, preventing potential failures), as depicted in \todo{\cref{xxx}}, which hinders the achievement of the desired ability.
%


%
% However, achieving this requires the robot to deeply understand the complex physical world and free-form human instructions, while accurately monitoring itself and the environment in real-time.
%

% Failure detection has advanced rapidly with the development of large language models~(LLMs)~\cite{dubey2024llama, touvron2023llama} and vision-language models~(VLMs)~\cite{achiam2023gpt, liu2024visual}.
% %
% Previous methods~\cite{liu2023reflect, shinn2023reflexion, yao2022react, ha2023scaling, huang2022inner, silver2024generalized, skreta2023errors, raman2022planning, du2023vision, liu2024self, zheng2024evaluating, duan2024aha, dai2024racer} employ LLMs with auxiliary vision modules or VLMs as post-execution failure detectors, neglecting in-execution detection.
% %
% To address this gap, recent works~\cite{guo2023doremi, yu2023multireact} frequently query VLMs during execution for failure detection. However, two major challenges remain: 1) detection isn't real-time due to the VLMs' high computational cost, and 2) it lacks precision, as VLMs exhibit limited 3D spatial understanding and frequent querying increases hallucination risks.
% %
% Moreover, these methods are reactive rather than proactive, detecting failures only after they occur and unable to prevent those arising from environmental changes or task modifications.
% %
% In this work, we study how to effectively endow robots with the ability to solve novel manipulation tasks specified by free-form language instructions using VLMs

%

The primary challenge in unifying proactive and reactive failure detection is finding a generalized modeling approach. We address this by formulating both tasks as spatio-temporal constraint satisfaction, verifying if entities (\eg, robots, object parts) achieve or maintain required states during or after execution to prevent and detect failures. To our knowledge, this is the first attempt to integrate both detection modes within a single framework. To enable real-time constraint satisfaction, we leverage VLM-generated code to compute inter-entity constraints and monitor their fulfillment, naming the framework Code-as-Monitor~({\fname}).

% To this end, we introduce Code-as-Monitor~({\fname}), a novel paradigm leveraging VLMs for both \textit{reactive} and \textit{proactive} failure detection via constraint-aware visual programming.  
%
% Our key idea involves two parts: 
%
% (1) We formulate \textit{reactive} and \textit{proactive} failure detection as generalized spatio-temporal constraint satisfaction, which involves checking if entities~(\eg, robots, object parts) in the scene maintain or reach the required states during or after execution, to prevent and detect failures. 
%
% (2) We employ the VLM-generated monitor code to compute inter-entity constraints in real-time, which reduces VLM calls~(\ie, generating code once per subgoal), thus minimizing hallucinations.

%
% Since direct visual programming from raw images and continuous monitoring remains challenging for VLMs, {\fname} is decomposed into two modules, \ie, the Painter and Monitor.
To improve the precision of constraint computation, we design two modules in {\fname}, \ie, the Painter and Monitor.
First, we leverage the painter to accurately extract the constraint elements~(\eg, points, lines, surfaces) and overlay them onto the image, as shown in the \cref{fig: motivation}~(c).
Instead of directly using the raw image for visual programming, we use the painter’s output as a visual prompt to improve precision.
%
% The Painter converts the textual constraints and current observations (\ie, multi-view RGB-D data) into constraint element proposals~(\eg, points, lines, surfaces) represented by 3D points and then annotated onto the images, as shown in the \cref{fig: motivation}~(c).
%
Notably, we train a multi-granularity constraint-aware segmentation model to obtain the constraint-related objects and parts, which can be lifted to 3D space using depth and better form the desired elements.
%
% Then the desired 3D points are selected from each part's point clouds to form the final elements compared to directly relying on 3D part segmentation models.
%
Second, the Monitor then translates these annotated images into monitor code and tracks these element positions in real-time, executing the code for both \textit{reactive} and \textit{proactive} failure detection.
%


%

% %
% Our key idea is to use VLMs to generate monitor code, enabling real-time checks on spatiotemporal constraints between entities (\eg, robots, object parts) during execution.
% %
% By computing the entity states and reducing the frequency of VLMs queries~(\ie, generating code once per subgoal), {\fname} improves precision and mitigates hallucinations.
%


% Direct visual programming from raw images remains challenging for VLMs, as it involves encoding both spatiotemporal states of entities and their constraints.
% %
% Thus, {\fname} is decomposed into two modules, as shown in \todo{\cref{xxx}}.
% %
% The first Painter, based on the current observations (\ie, multi-view RGB-D observations) and subgoals, generates textual constraints that are then annotated onto the images as constraint elements~(\eg, points, lines, surfaces), represented by 3D points in the world frame.
% %
% The second Monitor employs a VLMs (\eg, GPT-4o~\cite{achiam2023gpt}) to translate these annotated images into monitor code that specifies the state entities must maintain during and after subgoal execution.
% %
% It then continuously tracks the 3D points of the constraint elements in real time, executing the monitor code for immediate failure detection during execution.




% Notably, the Painter can autonomously generate constraint elements.
% %
% Specifically, our trained model performs constraint-aware part segmentation across multi-view images for each constraint. The segmented parts are then lifted to 3D space, with a representative 3D point selected from each part's point cloud. These points are then connected to form the final element of one constraint.
% %
% Compared to directly training a 3D part segmentation model, we can leverage more 2D image data for training, resulting in more accurate and generalizable performance.


%
We conduct extensive experiments in three simulators~(\ie, CLIPort~\cite{shridhar2021cliport}
, Omnigibson~\cite{li2022behavior}, and RLBench~\cite{james2019rlbench}) and one real-world setting, spanning diverse manipulation tasks (\eg, pick \& place, articulated objects), robot platforms (\eg, UR5, Franka, Fetch) and end-effectors (\eg, suction cup, gripper, dexterous hand).
%
The results show that {\fname} is generalizable and achieves both \textit{reactive} and \textit{proactive} failure detection in real-time, resulting in significantly higher success rates and reduced execution times compared to the baseline methods.
%
Moreover, {\fname} can quickly prevent potential failure caused by environment dynamics and human disturbance, enabling closed-loop planning in cluttered scenes.
%
Our contributions are summarized as follows:
\begin{itemize}
    \item We introduce Code-as-Monitor~(\fname), a novel paradigm that leverages VLMs for both \textit{reactive} and \textit{proactive} failure detection via constraint-aware visual programming.
    \item We propose a multi-granularity constraint-aware segmentation model to help obtain more precise constraint elements for generating more accurate monitor code.
    \item Extensive experiments show that {\fname} is generalizable and achieves more real-time and precise failure detection than baseline methods. 
\end{itemize}

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
